Clinical Prompt Learning with Frozen Language Models

Prompt learning is a new paradigm in the Natural Language Processing (NLP) field which has shown impressive performance on a number of natural language tasks with common benchmarking text datasets in full, few-shot, and zero-shot train-evaluation setups. Recently, it has even been observed that large but frozen pre-trained language models (PLMs) with prompt learning outperform smaller but fine-tuned models. However, as with many recent NLP trends, the performance of even the largest PLMs such as GPT-3 do not perform well on specialized domains (e.g. medical text), and the common practice to achieve State of the Art (SoTA) results still consists of pre-training and fine-tuning the PLMs on downstream tasks. The reliance on fine-tuning large PLMs is problematic in clinical settings where data is often held in non-GPU environments, and more resource efficient methods of training specialized domain models is crucial. We investigated the viability of prompt learning on clinically meaningful decision tasks and directly compared with more traditional fine-tuning methods. Results are partially in line with the prompt learning literature, with prompt learning able to match or improve on traditional fine-tuning with substantially fewer trainable parameters and requiring less training data. We argue that prompt learning therefore provides lower computational resource costs applicable to clinical settings, that can serve as an alternative to fine-tuning ever increasing in size PLMs. Complementary code to reproduce experiments presented in this work can be found at: https://github.com/NtaylorOX/Public_Clinical_Prompt.

==> tables/prompt_examples.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]
% \begin{table}[!htp]\centering
\caption{Example manual and mixed prompts for each clinical task. Note \textit{soft} tokens here represent the tunable continuous vectors or embeddings}\label{tab:prompt-examples}
\begin{tabular}{lrrrr}\toprule
\textbf{Task} &\textbf{Prompt type} &\textbf{Prompt template} & \\\midrule
ICD9 50 &manual &Patient has diagnosis {"mask"} & \\
& &Diagnosis is {"mask"}. & \\
&mixed &{"soft": "This"} patient {"soft":"has diagnosis"} {"mask"}. & \\
& & {"soft": "Diagnosis "} is {"mask"}. & \\
ICD9 triage &manual &Best department is {"mask"} & \\
& &Patient should go to department {"mask"}. & \\
&mixed &{"soft": "This"} patient {"soft":"should go to"} {"mask"}. & \\
& &{"soft": "This"} patient should {"soft":"go to this medical team based on symptoms of their illness"} {"mask"}. & \\
Mortality &manual &Patient is on the path to {"mask"}. & \\
& &Patient will be {"mask"}. & \\
&mixed &{"soft": "This"} patient {"soft":"on path to"} {"mask"}. & \\
& &patient will {"soft":"be"} {"mask"}. & \\
Length of stay &manual &The patient will be at hospital with a {"mask"} length. & \\
& &The length of stay of the patient will be {"mask"}. & \\
&mixed &{"soft": "This"} patient {"soft":"will be in hospital for a "} {"mask"} length. & \\
& &{"soft": "This"} patient {"soft":"will spend how long time in the hospital"} {"mask"}. & \\
\bottomrule
\end{tabular}
\end{threeparttable}\end{adjustwidth}
% \end{table}

==> tables/sensitivity_analysis.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with

%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}
%\centering
%\begin{threeparttable}[!htb]
\begin{table}[!htp]\centering
\caption{Number of trainable parameters vs performance across classification metrics.}\label{tab:sensitivity-analysis}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrrr}\toprule
\textbf{Paradigm} &\textbf{N params} &\textbf{Balanced accuracy} &\textbf{F1 weighted} &\textbf{AUC} \\\midrule
Traditional fine-tuning &1559 &0.2202 &0.3281 &0.7284 \\
&3887 &0.5442 &0.7526 &0.8989 \\
&7767 &0.1429 &0.0043 &0.6992 \\
&77607 &0.7914 &0.8794 &0.9771 \\
&\textbf{595975} &\textbf{0.8162} &\textbf{0.8919} &\textbf{0.98} \\
&626239 &0.5927 &0.7801 &0.9161 \\
&1552007 &0.8167 &0.8877 &0.9804 \\
\hline
Prompt learning &1536 &0.8128 &0.8995 &0.9757 \\
&3072 &0.8338 &0.9105 &0.9845 \\
&3840 &0.8351 &0.9089 &0.9838 \\
&9984 &0.8597 &0.9131 &0.9857 \\
&626536 &0.8367 &0.9166 &0.985 \\
&\textbf{628072} &\textbf{0.8698} &\textbf{0.9246} &\textbf{0.9889} \\
&628840 &0.8687 &0.9238 &0.9877 \\
&634984 &0.8654 &0.9193 &0.9866 \\
\bottomrule
\end{tabular}}
\end{table}
%\end{threeparttable}
%\end{adjustwidth}
